ELECTRE TRI-nB, pseudo-disjunctive: axiomatic and combinatorial results

ELECTRE TRI-nB is a method designed to sort alternatives evaluated on several attributes into ordered categories. It is an extension of ELECTRE TRI-B, using several limiting profiles, instead of just one, to delimit each category. ELECTRE TRI-nB comes in two flavours: pseudo-conjunctive and pseudo-disjunctive. In a previous paper we have characterized the ordered partitions that can be obtained with ELECTRE TRI-nB, pseudo-conjunctive, using a simple axiom called linearity. The present paper is dedicated to the axiomatic analysis of ELECTRE TRI-nB, pseudo-disjunctive. It also provides some combinatorial results.

==> ntheoremdefs.tex <==
\usepackage[centertags,reqno]{amsmath}
\usepackage{mathtools}
\usepackage[thmmarks,amsmath]{ntheorem}
    \RequirePackage{latexsym}
    \RequirePackage{amssymb}
    \theoremnumbering{arabic}
    \theoremstyle{break}
    \theoremsymbol{}
    \theorembodyfont{\itshape}
    \theoremheaderfont{\normalfont\bfseries}
    \theoremseparator{}
    %theorem, proposition, lemma, corollary, definition
\newtheorem{proposition}{Proposition}
\newtheorem{axiom}{Axiom}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{lemma}{Lemma}
    \theoremheaderfont{\normalfont\bfseries}%\slshape}
    \theorembodyfont{\upshape}
    \theoremsymbol{\ensuremath{\,\,\lrcorner}}
\newtheorem{definition}{Definition}
    \theoremsymbol{\ensuremath{\,\,\Diamond}}
    \theoremheaderfont{\normalfont\bfseries}%\slshape}
    \theorembodyfont{\upshape}
\newtheorem{example}{Example}
    \theoremheaderfont{\normalfont\bfseries}
    \theoremsymbol{\ensuremath{\ \bullet}}
\newtheorem{remark}{Remark}
\newtheorem{remTemp}{Temporary Remark}

\theoremstyle{nonumberbreak}
\theoremstyle{nonumberbreak}
\theorembodyfont{\normalfont}
\theoremsymbol{}
\newtheorem{tbd}{To be Done}
\newtheorem{convention}{Convention}
    \theoremheaderfont{\scshape}
    \theoremsymbol{\ensuremath{\ \Box}}
    \newtheorem{proof}{Proof}
    \newtheorem{pproof}{Partial proof}
    \theoremsymbol{}
    \theoremheaderfont{\normalfont\bfseries}
    \newtheorem{proofoflemma}{Proof of the lemma}
    \theoremsymbol{}
    \theoremheaderfont{\normalfont\bfseries}
    \newtheorem{claim}{Claim}
    \theoremsymbol{\par\hfill Fin Ajout}
    \newtheorem{ajout}{Ajout}
    \theoremclass{LaTeX}
    \newtheorem{question}{Question}

    \makeatletter
\newtheoremstyle{denisproof}%
  {\item[\rlap{\vbox{\hbox{\hskip\labelsep \theorem@headerfont
          ##1\theorem@separator}\hbox{\strut}}}]}%
  {\item[\rlap{\vbox{\hbox{\hskip\labelsep \theorem@headerfont
          ##1\ ##3\theorem@separator}\hbox{\strut}}}]}
\makeatother
\theoremstyle{denisproof}
    \theorembodyfont{\normalfont}
    \theoremheaderfont{\scshape}
\theoremsymbol{\ensuremath{\ \Box}}
\newtheorem{sproof}{Proof}

